MovieBench: A Hierarchical Movie Level Dataset for Long Video Generation

Recent advancements in video generation models, like Stable Video Diffusion, show promising results, but primarily focus on short, single-scene videos. These models struggle with generating long videos that involve multiple scenes, coherent narratives, and consistent characters. Furthermore, there is no publicly available dataset tailored for the analysis, evaluation, and training of long video generation models. In this paper, we present MovieBench: A Hierarchical Movie-Level Dataset for Long Video Generation, which addresses these challenges by providing unique contributions: (1) movie-length videos featuring rich, coherent storylines and multi-scene narratives, (2) consistency of character appearance and audio across scenes, and (3) hierarchical data structure contains high-level movie information and detailed shot-level descriptions. Experiments demonstrate that MovieBench brings some new insights and challenges, such as maintaining character ID consistency across multiple scenes for various characters. The dataset will be public and continuously maintained, aiming to advance the field of long video generation. Data can be found at: https://weijiawu.github.io/MovieBench/.

==> CustomizedVideoGen.tex <==
% \scriptsize
\begin{tabular}{l|cccc|ccc}
    \multirow{2}{*}{Method}  & \multirow{2}{*}{CLIP Score $ \uparrow $} & \multirow{2}{*}{Inception Score $ \uparrow $}  & \multirow{2}{*}{Aesthetic Score $ \uparrow $} & \multirow{2}{*}{FID $ \downarrow $ } & \multicolumn{3}{c}{${\rm  Character\,\,ID\,\,Consistency /\% \uparrow}$}  \\
    \cline{6-8} 
    & & & & & {${\rm  Precision_{ID} }$}  &  {${\rm  Recall_{ID} }$} & {${\rm  F1\,\,Score_{ID} }$}
    \\
    \hline
    Magic-Me~\cite{ma2024magic} &   &   &   &  &  &  & 
    
    % \whline
\end{tabular}

==> Metric.tex <==
% \def\x{{$\footnotesize \times$}}
% \scriptsize
% \setlength{\tabcolsep}{2pt}
\begin{tabular}{c|c|p{1.48\columnwidth}}
    % \whline
	Metric   & Better & Description   
    \cr
    % \shline \hline
	\hline

    % Character
    
   ${\rm  Portrait\,\,  Quality}$
   & higher  &  Quality assessment for character portraits, involving human raters scoring the image quality on a scale of 1 to 5, with 5 being the highest score. \cr \hline

    ${\rm  Portrait\mbox{-}Name\,\,Relevance}$
   & higher  &  Portrait-Name relevance score for each character name and portrait pair, with human raters on a scale of 1 to 5, and 5 being the highest score. \cr \hline
   
   ${\rm  Completeness}$
   & higher  &  Descriptive completeness score, assessing the extent to which the annotation of textual descriptions (\eg{} Plot, Background Description) reflects the completeness of the video content. \cr \hline

   ${\rm  Hallucination}$
   & lower  &  Fantasy score, assessing the degree of hallucination in textual descriptions of video content (e.g., Plot, Background Description). \cr \hline
   
   ${\rm  False\,\,  Postive(FP)}$
   & lower  &  The total number of false positives.  \cr \hline
   
    ${\rm  False\,\,  Negative(FN)}$
   & lower  & The total number of false negative. \cr \hline
   
   ${\rm  True\,\, Postive(TP)}$
   & higher  &  The total number of true positives. \cr \hline
   
    % ${\rm  True\,\, Negative(TN)}$
   % & higher  & The total number of true negatives. \cr \hline
   
   
   
   ${\rm  Recall}$
   & higher
   % & ICDAR2015(V), ICDAR2013(V), RoadText-1k, BOVText, DSText V1, DSText V2 
   & Ratio of correct detections\&recognitions to total number of GTs. Formula: $\frac{{\rm  TP}}{{\rm  TP} + {\rm  FN}}$ 
   \cr \hline
   
   ${\rm  Precision}$
   & higher 
    & Ratio of correct detections\&recognitions to total number of predicted detections\&recognitions. Formula: $\frac{{\rm  TP}}{{\rm  TP} + {\rm  FP}}$ 
    \cr \hline
    
    ${\rm F1\,\, Score}$ & higher 
   % & 
   % ICDAR2015(V), ICDAR2013(V), RoadText-1k,  BOVText, DSText V1, DSText V2 
   & ${\rm F1}$ Score~\cite{ristani2016performance}. The ratio of correctly identified detections\&recognitions over the average number of ground-truth and computed detections\&recognitions. Formula: $\frac{{\rm  Recall} \times {\rm  Precision} \times 2}{{\rm  Recall} + {\rm  Precision}}$    
   % \cr 
   % \hline
   % & ICDAR2015(V), ICDAR2013(V), RoadText-1k, BOVText, DSText V1, DSText V2 
     % \whline
\end{tabular}

